Unified Cross-modal Translation of Score Images, Symbolic Music, and Performance Audio

Music exists in various modalities, such as score images, symbolic scores, MIDI, and audio. Translations between each modality are established as core tasks of music information retrieval, such as automatic music transcription (audio-to-MIDI) and optical music recognition (score image to symbolic score). However, most past work on multimodal translation trains specialized models on individual translation tasks. In this paper, we propose a unified approach, where we train a general-purpose model on many translation tasks simultaneously. Two key factors make this unified approach viable: a new large-scale dataset and the tokenization of each modality. Firstly, we propose a new dataset that consists of more than 1,300 hours of paired audio-score image data collected from YouTube videos, which is an order of magnitude larger than any existing music modal translation datasets. Secondly, our unified tokenization framework discretizes score images, audio, MIDI, and MusicXML into a sequence of tokens, enabling a single encoder-decoder Transformer to tackle multiple cross-modal translation as one coherent sequence-to-sequence task. Experimental results confirm that our unified multitask model improves upon single-task baselines in several key areas, notably reducing the symbol error rate for optical music recognition from 24.58% to a state-of-the-art 13.67%, while similarly substantial improvements are observed across the other translation tasks. Notably, our approach achieves the first successful score-image-conditioned audio generation, marking a significant breakthrough in cross-modal music generation.

==> refs_supple.tex <==
\begin{thebibliography}{1}
\bibliographystyle{IEEEtran}
\bibitem{cocodataset}
T.-Y. Lin et al., ‘Microsoft COCO: Common Objects in Context’, in Computer Vision -- ECCV 2014, 2014, pp. 740–755.

\bibitem{esser2020taming}
P. Esser, R. Rombach, and B. Ommer, ‘Taming Transformers for High-Resolution Image Synthesis’, in Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR), 2021, pp. 12873–12883.

\bibitem{rodriguez2023ocr}
J. A. Rodriguez, D. Vazquez, I. Laradji, M. Pedersoli, and P. Rodriguez, ‘OCR-VQGAN: Taming Text-within-Image Generation’, in Proceedings of the IEEE/CVF Winter Conference on Applications of Computer Vision, 2023, pp. 3689–3698.

\end{thebibliography}


